HiGen: Hierarchy-Aware Sequence Generation for Hierarchical Text Classification

Hierarchical text classification (HTC) is a complex subtask under multi-label text classification, characterized by a hierarchical label taxonomy and data imbalance. The best-performing models aim to learn a static representation by combining document and hierarchical label information. However, the relevance of document sections can vary based on the hierarchy level, necessitating a dynamic document representation. To address this, we propose HiGen, a text-generation-based framework utilizing language models to encode dynamic text representations. We introduce a level-guided loss function to capture the relationship between text and label name semantics. Our approach incorporates a task-specific pretraining strategy, adapting the language model to in-domain knowledge and significantly enhancing performance for classes with limited examples. Furthermore, we present a new and valuable dataset called ENZYME, designed for HTC, which comprises articles from PubMed with the goal of predicting Enzyme Commission (EC) numbers. Through extensive experiments on the ENZYME dataset and the widely recognized WOS and NYT datasets, our methodology demonstrates superior performance, surpassing existing approaches while efficiently handling data and mitigating class imbalance. The data and code will be released publicly.

==> experiment_old.tex <==
\section{Experiments}
\subsection{Datasets}

\begin{table}[h!]
  \caption{Statistics of the Datasets used. $|L|$: total number target classes, $Depth$: level of the hierarchy, $Avg(|L_i|)$: Average number of classes per example.}
  \label{tab:data_statistics}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{lcccccc}
    \toprule
    Dataset & $|L|$ & Depth & $Avg(|L_i|)$ & Train & Val & Test \\
    \midrule
    ENZYME & 4,566 & 4 & 4 & 17,422 & 8,741 & 4,360  \\
    WOS & 141 & 2 & 2 & 30,070 & 7,518 & 9,397  \\
    NYT & 166 & 8 & 7.6 & 23,345 & 7,518 & 9397 \\
    \bottomrule
\end{tabular}
}
\end{table}

To evaluate the effectiveness of our model, we conduct experiments on three datasets for hierarchical text
classification following a single-path hierarchy. The first dataset is a newly proposed ENZYME dataset, which contains scientific documents in the Biomedical domain and the corresponding Enzyme Commission (EC) number of the enzyme each document talks about. We talk about this dataset in more detail in Section \ref{enzyme_dataset}. We release the training, validation and test splits for this dataset. Secondly, we chose the WOS dataset \cite{8260658} which includes abstracts of published papers from the Web of Science along with their corresponding labels organized in a hierarchy. We use the same training and testing splits used by \cite{zhou-etal-2020-hierarchy, chen-etal-2021-hierarchy, wang-etal-2022-incorporating}. Lastly, we use the Harvard USPTO Patent Dataset (HUPD) \cite{https://doi.org/10.48550/arxiv.2207.04043} that contains English-language utility patent applications filed to the United States Patent and Trademark Office (USPTO). We use the International Patent Classification (IPC) code as labels as they are hierarchical in nature. As proposed by the authors \cite{https://doi.org/10.48550/arxiv.2207.04043}, we only consider accepted patents since they contain reliable and accredited IPC codes. We use the same training and test splits from the dataset as proposed by the authors to evaluate our model against all the baselines. The statistics for all datasets are shown in Table \ref{tab:data_statistics}.

However, there exist more datasets for HTC. RCV1-V2 \cite{10.5555/1005332.1005345}, a news categorization corpora released by Reuters, Ltd; NYT \cite{nyt}, a news categorization corpora released by the New York Times; and EURLEX-57K \cite{chalkidis-etal-2019-large}, which contains English EU legislative documents. Since all these datasets have a multi-path hierarchical label structure, we do not evaluate the proposed model on them for now.

\subsubsection{\textbf{Pretraining Datasets}} 
\label{pretraining_dataset}
For the ENZYME dataset, we use the articles extracted from PubMed\footnote{\url{https://pubmed.ncbi.nlm.nih.gov/advanced/}}. We randomly sample 200,000 articles along with their Enzyme Commission (EC) numbers that follow a hierarchical structure. These articles are loosely labeled as they do not reflect human-annotated EC numbers. Both WOS and HUPD contain general-domain scientific documents from various fields. Hence, we use the arXiv dataset\footnote{\url{https://huggingface.co/datasets/arxiv_dataset}} for the in-domain pretraining as it contains documents of a similar nature. The arXiv dataset also has categories arranged in a hierarchical structure. 


\subsubsection{\textbf{ENZYME Dataset}}
\label{enzyme_dataset}
We propose a new dataset called ENZYME, which contains hand-curated full-text articles from the PubMed repository along with their Enzyme Commission (EC) numbers (see Section \ref{ec_system}) and enzyme names. The dataset contains 30,523 PubMed articles in both PDF and parsed formats. To our knowledge, no other dataset provides both full-text biomedical documents and the corresponding enzyme identification numbers. The EC numbers are organized in a hierarchy\footnote{\url{https://www.enzyme-database.org/contents.php}} and the statistics for each level are listed in Table \ref{tab:classes_per_level}. Unlike other datasets, the depth of hierarchical taxonomy for this dataset is 4, resulting in a large number of fine-grained classes and a complex hierarchical structure. Like with other HTC datasets, this dataset is highly imbalanced. Figure \ref{fig:data_statistics} shows a plot for the number of labels and the number of examples per label. From the figure \ref{fig:data_statistics} we can see that out of 4566 classes, $\sim$50\% have less than 2 examples. We only use the classes having 5 or more examples for our experiments. 

\begin{table}[h!]
  \caption{Number of classes per level in the ENZYME dataset}
  \label{tab:classes_per_level}
  \begin{tabular}{cc}
    \toprule
    Level & \# classes\\
    \midrule
    1 & 7\\
    2 & 24\\
    3 & 31\\
    4 & 462\\
    \midrule
    \# classes in the dataset: & 4566 \\ 
  \bottomrule
\end{tabular}
\end{table}

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.7\linewidth]{figures/fig4.pdf}
  \caption{ENZYME dataset statistics}
   \label{fig:data_statistics}
\end{figure}

\subsubsection{\textbf{Enzyme Classification (EC) System}}
\label{ec_system}
The Enzyme Commission (EC) number is a system for classifying enzymes, based on the chemical reactions they catalyze. The number is made up of four digits separated by periods and shows the enzyme's class, subclass, sub-subclass, and serial number respectively. This number is used to identify enzymes uniquely in the Enzyme Nomenclature database managed by the International Union of Biochemistry and Molecular Biology (IUBMB). The first digit (the "class" level) defines one of seven major enzymatic reaction types, e.g., hydrolases that use water to break a chemical bond. The second (the "subclass" level) and third digits (the "sub-subclass" level) represent more specific reaction types within their parent (sub-)class. The fourth digit (the "serial number" level) is a unique identifier assigned to a specific enzyme, usually determined by a specific substrate. For example, the enzyme number EC 1.3.8.2 represents an enzyme in class 1 (Oxidoreductases), subclass 3 (Acting on CH-CH group of donors), sub-subclass 8 (With a flavin as acceptor) with a unique number 2 (to identify a specific substrate 4,4'-diapophytoene).

\subsubsection{\textbf{Construction}}
The BRENDA database \cite{chang2021brenda} was parsed to collect enzymes with both EC number definitions and PubMed references. Following an inspection of retrieved entries, we downloaded the freely available PDFs for each of the articles from PubMed. To extract well-formatted text from these files, we used an open-source tool called SciPDFParser\footnote{\url{https://github.com/titipata/scipdf_parser}}. For this work, we use the title, abstract and introduction sections from each paper.

\subsection{Experimental Setup}
\subsubsection{\textbf{Baselines}}
To compare the proposed method, we select a few recent baselines. HGCLR \cite{wang-etal-2022-incorporating}, HiMatch \cite{chen-etal-2021-hierarchy} and HiAGM \cite{zhou-etal-2020-hierarchy} label and text encoding modules to learn the joint representation for hierarchical text classification. We implemented BERT based encoding model for the HiMATCH model. HGCLR inherently uses BERT based encoder model. As our proposed approach contains a novel pretraining objective and the constraint decoding strategy, we compared the proposed approach with a Vanilla model (without pretraining and constraint decoding strategy).

We compare our method with a classic BERT-based text classification model. In order to incorporate hierarchy into the BERT classification, we add linear layers corresponding to each layer in the hierarchy. Based on the number of hierarchies in the dataset, different linear layers are added on top of the BERT encoder. The number of classes in each linear layer is decided based on the number of classes for that level in the dataset. This is precomputed and fixed for a dataset.

\begin{table*}[t!]
  \label{tab:comparison}
  \begin{tabular}{lcccccc}
     \toprule
     \multirow{2}{*}{Models} & \multicolumn{2}{c}{ENZYME} & \multicolumn{2}{c}{WOS} & \multicolumn{2}{c}{HUPD} \\
     \cline{2-7}
     & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1  \\
    \midrule
    BERT & 70.22  & 51.97  & 74.30 &	76.84 & 62.89 &	35.29 \\
    HiAGM & 40.57 & 36.95  & 74.02 &	81.71 & 51.14  &	31.80\\
    HiMATCH & 54.95 & 51.86  & 73.41 &	81.30 & - & -\\
    BERT + HiMATCH & 58.24 & 56.31  & 77.93 & \textbf{84.40} & - & - \\
    HGCLR &  70.71 & 67.71  & 76.42 &	81.32 & 55.35  &	36.59\\ \midrule
    \rowcolor{gray!10}  \textbf{HiGen (Ours)} & \textbf{85.57} & \textbf{81.64}  & \textbf{81.40} & 80.66 & \textbf{66.01} &	\textbf{44.56} \\
    \bottomrule
    \caption{Experimental results of our proposed approach on all datasets. For a fair comparison, we implemented all the baselines with the proposed evaluation metric.}
\end{tabular}
\end{table*}



\subsubsection{\textbf{Implementation Details}}
We employ different checkpoints of the BART model as the starting point, depending on the dataset. For the ENZYME dataset, we utilize a BART model that has been fine-tuned on PubMed articles\footnote{mse30/bart-base-finetuned-pubmed}, while for WOS \& HUPD, we use a BART model that has been fine-tuned on ArXiv articles\footnote{mse30/bart-base-finetuned-arxiv} from Huggingface. Using these models, we first apply the proposed pretraining strategies and further pretrain on the data collected in Section \ref{pretraining_dataset} and save the resulting checkpoints. These are subsequently fine-tuned on the ENZYME, WOS \& HUPD datasets for the task of HTC. We use a batch size of 4 for both the pretraining and fine-tuning stages. We utilize the Adam optimizer, with an initial learning rate of 5e-5 and a linear learning rate scheduler.
% Our results are reported on the test sets of all datasets. 
To implement constrained decoding, we set the logits at each decoding step to a large negative value ($-\infty$) with the exception of a fixed set of allowed tokens. The set of permitted tokens is dynamic and varies based on the level of the data hierarchy. The token with the highest score is then chosen as the prediction for the corresponding decoding step. For the baselines (HiAGM, HiMatch, \& HGCLR), we use the implementations provided by the authors to produce results on all datasets. The BERT baseline model is initialized with the BERT pretrained on PubMed articles\footnote{microsoft/BiomedNLP-PubMedBERT-base-uncased-abstract-fulltext} for the ENZYME dataset. Similarly, we use the base-BERT\footnote{bert-base-uncased} for the HUPD and WOS datasets.
The hyperparameters of all models are tuned on the validation set from all datasets. All models were implemented using PyTorch.

\subsubsection{\textbf{Evaluation Strategy}}
The evaluation strategy used by all previously proposed approaches flattens the hierarchy and treats all nodes as if they are leaf nodes, like in multi-label classification. This evaluation technique does not impose any constraints on the number of labels that needs to be present in the final classification. A threshold of 0.5 is chosen to select all classes having softmax probabilities greater than it as the final prediction of the classes in the hierarchy. 
This approach has two main drawbacks: first, it ignores the hierarchical structure and treats all nodes as equal during evaluation, and second, there is no way to track the path taken by the model through the hierarchy from the root to the leaf class.

To address the limitations of previous evaluation strategies for hierarchical text classification (HTC), we propose a new evaluation method. Our approach focuses on the path taken by the model from the root node to the leaf node in order to make the final classification. This new evaluation strategy is more stringent compared to previous methods as it ensures the accuracy of the entire path. As an example, if the ground truth label and the predicted output from the model are:
\begin{align*}
\text{Ground truth}: X \rightarrow Y \rightarrow Z \rightarrow W  \\
\text{Model prediction}: X \rightarrow Y \rightarrow Z \rightarrow K
\end{align*}

Under our evaluation method, this would be considered incorrect. In addition to the path-based evaluation, our evaluation approach also evaluates the level-wise prediction efficiency of the model, comparing it to the baseline models using the same evaluation criteria. This allows us to assess the model's performance at each level of the hierarchy, even if the final prediction is incorrect.

\subsubsection{\textbf{Evaluation Metrics}}
We evaluated the performance of our model using the evaluation strategy outlined in the previous section, which takes into account the correctness of the entire path through the hierarchy. Partial correctness is considered a failure. The standard evaluation metrics Micro-F1 and Macro-F1 were used to capture this information, as these metrics are widely accepted in the field \cite{10.1145/2487575.2487644}.
The Macro-F1 score computes the average F1 score giving equal weight to each class. The Micro-F1 score, on the other hand, calculates the global F1 score by summing up the true positives, false positives, and false negatives. It is important to consider both metrics to fully evaluate the performance of a model.
% Given that all datasets used in this study were imbalanced, with some classes having very few training and test examples, the Micro-F1 score was given more importance in our evaluation.

\begin{table*}[t!]
  \caption{Experimental results for the level-wise performance of our proposed approach and baselines on the ENZYME dataset. We used the same proposed evaluation strategy for a fair comparison.}
  \label{tab:level_wise}
  \begin{tabular}{lcccccc}
     \toprule
     \multirow{2}{*}{Models} & \multicolumn{2}{c}{Till Level 1} & \multicolumn{2}{c}{Till Level 2} & \multicolumn{2}{c}{Till Level 3} \\
     \cline{2-7}
     & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1  \\
    \midrule
    BERT & 96.07 & 94.78 & 93.76 & 81.84 & 90.29 & 76.97 \\ 
    HiAGM & 88.14 & 77.56 & 77.47 & 68.12 & 68.36 & 59.05 \\ 
    HiMatch & 82.11 & 71.72 & 65.82 & 58.03 & 55.22 & 48.83 \\ 
    HGCLR & 95.22 & 82.81 & 91.67 & 88.96 & 87.67 & 84.89 \\ 
    Vanilla BART & 95.43 & 94.01 & 92.36 & 87.52 & 88.48 & 81.07 \\  \midrule
    \rowcolor{gray!10} \textbf{HiGen (Ours)} & \textbf{96.33} & \textbf{95.13} & \textbf{94.90} & \textbf{92.63} & \textbf{93.14} & \textbf{89.80} \\ 
    \bottomrule
\end{tabular}
\end{table*}

\subsection{Main Results}
The results of our study and baselines are summarized in Table \ref{tab:comparison}. Our model, HiGen, consistently outperforms all previous approaches across all datasets. The simplicity of the model and its effective pretraining strategy allow it to attend to relevant details of the document while predicting the class of any level, thereby generating a coherent class hierarchy. 
To ensure a \emph{fair comparison} among baseline models using BERT-based encoders and HiGen, we made sure to initialize each model according to the dataset. For example, the BERT encoder in HGCLR was initialized with the PubMed BERT model for the ENZYME dataset. Our model outperforms HGCLR on both ENZYME and HUPD datasets, achieving substantial performance gains.
Compared to other approaches, HiGen performs better on deep and complex label hierarchies, particularly on the ENZYME dataset. On this dataset, our model demonstrates a 13.77\% and 11.72\% improvement in Micro-F1 and Macro-F1 scores, respectively, over the HGCLR model. The BERT baseline, which was finetuned on PubMed articles, outperforms other baselines like HiAGM and HiMatch, leading to its high performance.

We observe a similar trend on HUPD as HiGen improves upon HGCLR by 10.66\% and 8\% on the Micro-F1 and Macro-F1 scores. 
With HiGen's pretraining task being very similar to the finetuning objective, it helped in leveraging the encoded hierarchical information effectively. On the WOS dataset, HiGen showed a moderate improvement on the Micro-F1 score, but the performance gains were not as substantial as the other datasets. This can be attributed to the simple hierarchical structure of the WOS dataset  (Table \ref{tab:data_statistics}). We achieve an improvement of about 3\% only on the Micro-F1 score from HiMatch-BERT while previous approaches perform better on the Macro-F1 score. Overall, HiGen demonstrates an impressive ability to encode complex and deep label hierarchies.

\subsection{Level-wise Performance}
The evaluation strategy assesses the accuracy of the entire predicted label for hierarchical classification. If there is an error at any level, it is deemed a misclassification. To evaluate the model's ability to predict a hierarchical label, it is further scrutinized by examining its performance at intermediate levels of the hierarchy. For example, in the ENZYME dataset, there is a four-level deep hierarchy. Hence, the evaluation strategy examines the performance of the model at depths 1, 2, \& 3. The baseline methods are evaluated by choosing the predicted class up to the given depth, and the performance is recorded using the Micro-F1 and Macro-F1 scores at each level.

Table \ref{tab:level_wise} displays the results of the level-wise performance of HiGen and various baseline methods on the ENZYME dataset. The performance of the model decreases as the depth of the hierarchy increases. At Level 1, the performance is high, $\sim$90\%, because there are very few classes, but as the depth increases to Levels 2 and 3, the performance drops due to an increase in the number of plausible classes. While comparing the decrease in performance of the models from Level 1 to Level 3, HiGen decreases by 3.31\% for the Micro-F1 score whereas the best-performing baseline, HGCLR, decreases by 10.84\%. For the BERT baseline, the decrease in performance is 6.07\%. Performance results for the full depth of the hierarchy, up to Level 4, are presented in Table \ref{tab:comparison}. The superior performance justifies that HiGen can better understand \& exploit the hierarchical structure of the labels, which leads to robust performance over all levels.

\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/longtailed_micro.pdf}
         \caption{Micro-F1 v/s Frequency of Classes}
         \label{fig:longtailed_micro}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/longtailed_macro.pdf}
         \caption{Macro-F1 v/s Frequency of Classes}
         \label{fig:longtailed_macro}
     \end{subfigure}
     \caption{Performance on ENZYME dataset for the long-tailed classes}
     \label{fig:longtailed}
\end{figure}


\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=0.49\linewidth]{figures/limited_biomed_micro.pdf}
         \hfill
         \includegraphics[width=0.49\linewidth]{figures/limited_biomed_macro.pdf}
         \caption{Dataset: ENZYME}
         \label{fig:limited_biomed}
     \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.24\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figures/limited_biomed_macro.png}
     %     \caption{Macro-F1 v/s Training Data Fraction}
     %     \label{fig:limited_biomed_macro}
     % \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=0.49\linewidth]{figures/limited_wos_micro.pdf}
         \hfill
         \includegraphics[width=0.49\linewidth]{figures/limited_wos_macro.pdf}
         \caption{Dataset : WOS}
         \label{fig:limited_wos}
     \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.24\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figures/limited_wos_macro.png}
     %     \caption{Macro-F1 v/s Training Data Fraction}
     %     \label{fig:limited_wos_macro}
     % \end{subfigure}
     \caption{Performance for test sets of ENZYME \& WOS datasets on varying the training data proportion.}
     \label{fig:limited}
\end{figure*}


\subsection{Performance on Long-Tailed Distribution}
 As we know the datasets used in the experiment suffer from significant data imbalance. A majority of classes have only a small number of examples for training and testing. For instance, in the ENZYME dataset, out of 1482 classes, 670 classes have fewer than 10 examples in the entire dataset. These classes with limited examples are referred to as \emph{long-tailed classes}. Judging performance on these \emph{long-tailed classes} is crucial as it reflects the model's ability to learn from limited training data and provides insight into the model's robustness and generalization capabilities.

 We evaluate the performance of the models on the long-tailed classes by dividing the testing data into bins based on the frequency of the classes appearing in the testing data. These bins range from 1 to 5. Figure \ref{fig:longtailed} shows the results for the ENZYME dataset, with Micro-F1 (Figure \ref{fig:longtailed_micro}) and Macro-F1 (Figure \ref{fig:longtailed_macro}) scores plotted against the frequency of the classes. The models compared are the BERT-based classifier (HGCLR), Vanilla BART, and HiGen. Our proposed approach, HiGen, outperforms all baseline models on both metrics, across all frequency bins of the test classes. It is worth noting that a stratified sampling split was used for the entire dataset, meaning that classes with few examples in the test split also have few examples in the training split. The bins were created based on the frequency of classes in the test split for ease of representation and simplicity.
The performance of HiGen surpasses the best baseline (HGCLR) by a substantial margin, with an improvement of at least 20 points for the Micro-F1 score and 15 points for the Macro-F1 score for all class frequencies. The excellent performance of HiGen is attributed to its pretraining strategy and the constraint decoding mechanism used.


\subsection{Data Efficiency}


To test the robustness of our model we trained it on various portions of the input data and evaluated its performance on the original test set. This experiment was also conducted on several baseline models for a fair comparison. These baselines include BERT as a simple baseline, HGCLR, which is the best-performing baseline available publicly, and Vanilla BART to assess the improvement brought by our pretraining and constraint decoding strategies. The results of this analysis for both the ENZYME and WOS datasets are shown in Figure \ref{fig:limited}. Each curve in the figure represents the performance of each model on the test set as the amount of training data increases.

Our approach was found to outperform all baseline models for the ENZYME dataset, as seen in Figure \ref{fig:limited_biomed}. Even when trained on only 10\% of the training data, our model showed remarkable performance on the test set. This is in contrast to the second-best performing model, a vanilla PubMed BART\footnote{mse30/bart-base-finetuned-pubmed} model, which was trained on the same 10\% of the training data. Our high performance can be attributed to the knowledge gained during the pretraining stage, where the model was asked to predict labels for certain levels given the input text and other parts of the hierarchical label. This embeds information about the label hierarchy into the model without the need for complex graphical encoders, unlike in HiAGM, HiMatch, and HGCLR.

On the WOS dataset (as shown in Figure \ref{fig:limited_wos}), we also observe a strong performance by our model, especially when trained with limited data. While the Vanilla ArXiv BART\footnote{mse30/bart-base-finetuned-arxiv} and BERT models also perform well when trained with only 10\% of the data, all models tend to have similar performance when trained with more data. This could be due to the inherently simple class hierarchy structure of the WOS dataset, which is characterized by a two-level hierarchy with a small number of labels. In contrast, the poor performance of HGCLR in low data settings could be attributed to its contrastive training nature, which requires a larger amount of data. This is evident from the noticeable improvement in performance as we increase the proportion of data for training.

\subsection{Ablation Study}

\begin{table}[t!]
  \label{tab:ablation}
  \begin{tabular}{lcc}
    \hline
    Model & Micro-F1 & Macro-F1\\
    \hline
    Vanilla BART & 86.26 & 79.34 \\
    HiGen & \textbf{87.39} & \textbf{81.54} \\
    \hspace{3mm}w/o pretraining & 86.69 & 80.54 \\
    \hspace{3mm}w/o $\mathcal{L}_{O}$ & 87.35 & 81.11 \\
    \hspace{3mm}w/o $\mathcal{L}_{T}$ & 87.19 & 80.83 \\
    \hspace{3mm}w/o $\mathcal{L}_{S}$ & 87.33 & 80.91 \\
    \hline
\end{tabular}
\caption{Performance on removing some components of HiGen on the test set of WOS.}
\end{table}

\textbf{Vanilla BART} For this experiment, we directly train the BART-base model using just the language modeling loss. We train this model on the same training data followed by evaluation on the test set. The result, as shown in Table \ref{tab:ablation}, indicates a significant decline of 1.13 and 2.2 points in Micro-F1 and Macro-F1 scores from HiGen. These results demonstrate the impact of the proposed innovations.

\textbf{Without Pretraining:} In this experiment, we removed the pretraining strategy from HiGen, resulting in a BART-base model trained with all the proposed loss functions. The result shown in Table \ref{tab:ablation}, indicates a drop in performance with a decrease of 0.7\% in the Micro-F1 score and 1\% in the Macro-F1 score. These results demonstrate that the pretraining strategy is crucial for achieving better performance and that weakly labeled data generated using powerful LLMs can be utilized as a good source for this task.

\textbf{Without Output Space Loss:} In this experiment, we remove $\mathcal{L}_{O}$ from the training objective. We observe a slight reduction in performance from HiGen with a larger effect on the Macro-F1 score [write some reason for this].

\textbf{Without Token Constraint Loss:} In this experiment, we remove $\mathcal{L}_{T}$ from the training objective. We observe a considerable drop in performance from HiGen on both metrics. This indicates that restricting the model to the set of allowed tokens actually helps boost performance. [improve reason]

\textbf{Without Level-Guided Semantic Loss:} In this experiment, we remove $\mathcal{L}_{S}$ from the training objective. We observe a slight reduction in performance from HiGen on the Micro-F1 score but a considerable drop on the Macro-F1 score. [write reason for this]

The removal of certain components in the proposed approach led to a significant decrease in performance.

% \subsection{Ablation Study}

% \begin{table}[t!]
%   \caption{Performance on removing some components of HiGen on the test set of WOS.}
%   \label{tab:ablation_1_1}
%   \begin{tabular}{lcc}
%     \toprule
%     Model & Micro-F1 & Macro-F1\\
%     \midrule
%     Vanilla BART & 86.26 & 79.34 \\
%     HiGen & \textbf{87.39} & \textbf{81.54} \\
%     \hspace{3mm}w/o Pretraining & 72.04 & 60.84 \\
%     \hspace{3mm}w/o Output Space Loss & 79.58 & 73.18 \\
%     \hspace{3mm}w/o Token Constraint Loss & 85.07 & 80.37 \\
%     \hspace{3mm}w/o Level-guided Semantic Loss & 85.07 & 80.37 \\
%     \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[h!]
%   \caption{Performance on removing some components of HiGen on the test set of WOS.}
%   \label{tab:ablation_1_2}
%   \begin{tabular}{lcc}
%     \toprule
%     Model & Micro-F1 & Macro-F1\\
%     \midrule
%     Vanilla BART & 78.69 & 79.12 \\
%     HiGen & \textbf{81.40} & \textbf{80.66} \\
%     \hspace{3mm}w/o Pretraining & 80.99 & 80.06 \\
%     \hspace{3mm}w/o ArXiv BART & 81.03 & 80.21 \\
%     \hspace{3mm}w/o CD & 80.15 & 78.73 \\
%     \bottomrule
% \end{tabular}
% \end{table}

% To assess the effect of each component in our proposed method, we conduct experiments where we eliminate certain elements and measure the performance. This allows us to determine the contribution of each component to the performance of HiGen and understand the significance of each element in the approach.


% \textbf{Vanilla BART:} For this experiment, we used the original BART model without any initialization, proposed pertaining, or constrained decoding. We train this BART model on the training data followed by evaluation on the test set. The results, as shown in Tables \ref{tab:ablation_1_1} \& \ref{tab:ablation_1_2}, indicate a significant improvement of 18 and 26 points on Micro-F1 and Macro-F1 scores respectively for the ENZYME dataset and a slight improvement for the WOS dataset.  These results demonstrate the impact of the proposed innovations.

% \textbf{Without Pretraining:} In this experiment, we removed the pretraining strategy from our proposed model, resulting in a Vanilla BART model initialized with PubMed BART for the ENZYME dataset and ArXiv BART for the WOS dataset, followed by constrained decoding. The results, as shown in Tables \ref{tab:ablation_1_1} and \ref{tab:ablation_1_2}, indicate a drop in performance with an average decrease of 6.97\% in the Micro-F1 score and 10.7\% in the Macro-F1 score. These results demonstrate that the pretraining strategy is crucial for achieving better performance and is a critical component of the proposed approach. Since our pretraining task is similar to the actual finetuning task, it allows the model to learn effectively, which contributes to improved performance.

% \textbf{Without a pre-initialized BART model:} In this experiment, the only alteration made was to the initialization of the BART model. Instead of using the domain-specific PubMed or ArXiv BART, the BART-base (from HuggingFace's facebook/bart-base) was used for both datasets. The use of a domain-specific pretrained model provides a strong foundation of domain knowledge, which saves data and computational resources needed for training on a specific task. The results showed a decline in performance, with an average decrease of 3.18\% observed in the Micro-F1 score and 4.46\% in the Macro-F1 score.

% \textbf{Without Constraint Decoding:} To validate the effectiveness of the constrained decoding (CD) step, the proposed model was tested without CD during inference. The results showed that the addition of CD enhances the performance of the model by an average of 0.88\% in the Micro-F1 score and 1.6\% in the Macro-F1 score.

% The removal of certain crucial components of the proposed approach had a significant impact on performance, with the effects being more pronounced on the ENZYME dataset than on WOS. This disparity is likely due to the simplicity of the WOS label hierarchy, making it easier for basic models to learn. Through this ablation study, we have demonstrated the significance of each component in the proposed approach and their contribution to improved results in a setting with a complex hierarchy and limited data. The proposed pretraining step and the constrained decoding step are crucial and essential components of the proposed approach and play a key role in achieving better performance.

The removal of certain components in the proposed approach led to a significant decrease in performance, with the impact being greater on the ENZYME dataset than on WOS. This disparity can be attributed to the simplicity of the WOS label hierarchy, making it easier for basic models to learn. Through this ablation study, we demonstrate the importance of each component in the proposed approach, and it was found that the pretraining step and the constrained decoding step are crucial and necessary for improved results in a scenario with a complex hierarchy and limited data.

==> intro.tex <==
\section{Introduction}
Hierarchical text classification (HTC) aims to classify text data into predefined categories  organized in a hierarchical structure~\cite{banerjee-etal-2019-hierarchical,wang-etal-2022-incorporating,zhou-etal-2020-hierarchy}, which serves as a fundamental task for text mining with various applications such as 
scientific paper recommendation~\cite{zhang2020multi}, 
semantic indexing~\cite{li2019hiercon}, and online advertising~\cite{agrawal2013multi}.
In HTC, the hierarchy often comprises multiple levels, each with its own set of categories or classes. The goal is to accurately assign a text document to the most appropriate category or class at each level of the hierarchy, based on its content and characteristics. \yue{this sentence is redundant has you mentioned this in the first sentence.} In contrast to the classical text classification task, HTC is inherently complex because of the huge imbalance of data at different levels and learning the dependency between levels. 

Figure \ref{fig:teaser} shows the hierarchical structure represented as a tree which is encoded in the model to generate the final hierarchal label. From the taxonomy tree it can be observed that as the depth increases, the number of classes grows exponentially leading to a huge imbalance in the data. \yue{I don't understand why there is an imbalanced issue. If each node contains the same amount of documents, then the dataset is actually balanced.}
There exists various datasets like WOS \cite{8260658}, Harvard USPTO Patent Dataset (HUPD) \cite{https://doi.org/10.48550/arxiv.2207.04043}, RCV1-V2 \cite{10.5555/1005332.1005345}, NYT \cite{nyt}, and EURLEX-57K \cite{chalkidis-etal-2019-large} having a hierarchical taxonomy for labels. \yue{Why mentioning these datasets without actually using them in the experiments?} But these datasets have an overall limited number of classes, thereby having a shallow hierarchy. Real-world HTC applications often involve more complex taxonomies with deeper label structures and numerous classes with limited examples. These characteristics can lead to performance degradation for existing HTC methods.

% Figure 1 shows the hierarchical taxonomy existing in the label set. As the depth in the hierarchy increases, the number of classes grows exponentially leading to a huge imbalance in the data. Based on the type of dataset used for the problem, HTC can be categorized into single-path and multi-path hierarchies. In the single-path hierarchy, only one unique path to the leaf label is possible (Figure 1). On the other hand, for multi-path hierarchy, labels could have multiple paths from the root node to the leaf node. In this paper, we will look into the single-path hierarchical text classification.

% There are various datasets like WOS \cite{8260658}, Harvard USPTO Patent Dataset(HUPD) \cite{https://doi.org/10.48550/arxiv.2207.04043}, RCV1-V2 \cite{10.5555/1005332.1005345}, NYT \cite{nyt}, and EURLEX-57K \cite{chalkidis-etal-2019-large} used for HTC. WOS and HUPD are single-path hierarchical dataset whereas  RCV1-V2, NYT, and EURLEX-57K are multi-path hierarchical dataset. The available single-path hierarchical dataset has a limited number of hierarchies and very few labels. We propose an ENZYME dataset that contains complex hierarchical depth and a larger number of hierarchical labels making it more complex. \yy{This paragraph is a bit abrupt, and does not well support your contribution. You may need to further emphasize the difficulty of the newly proposed dataset.}


% Specifically, existing methods for hierarchical text classification (HTC) can be categorized into two groups: global \cite{zhou-etal-2020-hierarchy, chen-etal-2021-hierarchy} and local \cite{shimura-etal-2018-hft, banerjee-etal-2019-hierarchical, wehrmann2018hierarchical}.
% Global models  transform the hierarchy into a flat structure followed by a single classifier for all the classes.
% Some global models utilize Graph Convolution Networks (GCN) \cite{zhou-etal-2020-hierarchy}, TreeLSTMs \cite{zhou-etal-2020-hierarchy}, Label correlation features \cite{lu-etal-2020-multi}, hierarchical regularization \cite{10.1145/2487575.2487644}, and meta-learning \cite{wu-etal-2019-learning}.
% Local models XXX
%  utilizes the hierarchical structure in a top-down manner \zc{this summary is not detailed enough} .
% This kind of model suffers from two major drawbacks.
% Firstly, it increases the number of classes in the classifier exponentially, which results in highly imbalanced data.
% Secondly, these methods capture the dependencies between hierarchical classes in a very limited manner.
% These methods rely heavily on the label semantics and the dependency between different nodes in the hierarchy to encode richer information, making them heavily complex.
%  \zc{I think this paragraph needs to be improved. You first summarize global and local methods, and then point out the issues  all of them suffer from. Focus on the issues that our method can address. For example, they do not model the dependency very well (but our sequence to sequence pretraining and generating can do that ); they do not handle long-tail distribution very well (but later we sell that our method can address that)} 

Specifically, existing methods for hierarchical text classification (HTC) can be categorized into two groups: global \cite{zhou-etal-2020-hierarchy, chen-etal-2021-hierarchy} and local \cite{shimura-etal-2018-hft, banerjee-etal-2019-hierarchical, wehrmann2018hierarchical}. The local method approaches the problem by building multiple classifiers for different levels and utilizes the hierarchical structure in a top-down manner. Global models, on the other hand,  transform the hierarchy into a flat structure followed by a single classifier for all the classes. Some global models utilize Graph Convolution Networks (GCN) \cite{zhou-etal-2020-hierarchy}, TreeLSTMs \cite{zhou-etal-2020-hierarchy}, Label correlation features \cite{lu-etal-2020-multi}, hierarchical regularization \cite{10.1145/2487575.2487644}, and meta-learning \cite{wu-etal-2019-learning}. This group of models suffer from two major drawbacks. Firstly, it increases the number of classes in the classifier exponentially, which results in highly imbalanced data. Secondly, these methods capture the dependencies between hierarchical classes in a very limited manner. \yue{These two drawbacks mentioned here are very hand-waving. For example, I feel that using GCNs can  encode label relationships. Also, the drawbacks of using discriminative language models can be mentioned. e.g. they don't fully understand the label semantics} Because of these limitations, the aforementioned models suffer significantly in their performance for long-tailed classes i.e. classes with very limited data in the training set.



\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/overview.pdf}
  \caption{A hierarchical text classification example}
   \label{fig:teaser}
\end{figure}

We propose to fully unleash the power of large pretrained language models (PLM) in solving the task of hierarchical text classification.
Notably, these language models are pretrained on massive collections of text data with diverse topics, allowing them to encode generic linguistic features that can be transferred across different tasks~\cite{liu2019linguistic}. 
We transform the problem of HTC to a text generation problem using a generative model built using the transformer-based Sequence-to-Sequence (Seq2Seq) framework~\cite{lewis-etal-2020-bart}.
This framework captures the entire hierarchy in an autoregressive manner by generating a label for the current level conditioned on the previous ones. This approach allows the model to effectively capture complex dependencies between the encoded document and the current label hierarchy and leverage them to correctly predict the label at the next level. 
 % \zc{you should elaborate  the discussion: how this generation can address the challenges mentioned earlier } 

Inspired by the success of effective pretraining tasks~\cite{gururangan2020don}, we propose a task-related pretraining strategy for this generation-based model.
The aim of this pretraining strategy is to jointly learn a representation for the text and label to capture the dependencies amongst them.
This pretraining step is performed on additional weakly-labeled data from the same domain as the original data, thereby creating a domain-specific pretrained model. As described in \cite{mueller2022label, gururangan2020don}, having access to this in-domain knowledge helps the pretrained model in dealing with the issue of a huge data imbalance, which is an inherent problem in an HTC dataset. \yue{It is too high-level, and after reading this paragraph, it seems that you directly use the existing approach for continuous pretraining, which is not very interesting.}
Additionally, we implement a constrained decoding strategy to ensure the generation of coherent hierarchical labels by limiting any unnecessary labels\yue{what do you mean by unnecessary?} being generated during the decoding phase.


% \zc{each paragraph makes one point please, if you are selling the strength of the method, then just focus on that. The experiment findings can be discussed in another paragraph, in a more detailed way.}
%  \zc{again, when talking about pretarinng, focus and elaborate on why it is novel and flexible, why it addresses the challenges. And you should also talk about the constrained decoding mechanism and its benefits here too.} 


%  \zc{expand the experiment like this: we have performed experiments on XXX datasets with diverse characteristics; we find our method outperforms the strongest baselines by XX to XXX; we also find it excels in XXX situations} 
% Our model outperforms the baseline models on average by 10\% on the proposed metrics, even when experimented with classes having very limited examples. None of the past works on HTC explores the use of relevant data for the pretraining task. 

% The pretraining strategy helps the model capture more domain-specific knowledge using some weakly supervised data.  \yy{The weakly-supervised data here is abrupt and unclear. How is the weakly supervised data collected? How do you leverage these weak labels?}

% Having access to larger domain-specific knowledge helps the model handle the inherent problem of huge data imbalance in the dataset. \yy{why? I cannot see a clear connection between these two terms.}
% Our model outperforms the baseline models by incorporating more comprehensive information, even when there are limited samples for most of the classes. 
% \yy{It is better to calculate the relative gain here.}
% None of the past works explores the importance of using relevant data for the pretraining task and showcases the benefits of such a strategy on low-resource classes. \yy{Be cautious with claims such as 'None of the past works explores', I don't think it is true. Pretraining benefits low-resource classification have been discussed in papers such as "Label Semantic Aware Pre-training for Few-shot Text Classification", "Don't Stop Pretraining: Adapt Language Models to Domains and Tasks", "Multi-stage pre-training for low-resource domain adaptation".}


% In this work, we propose a new hierarchical dataset from the field of biomedicine \zc{don't focus on the dataset, we are solving the general hierarchical classification problem. Use the first paragraph to state why the problem is important.} . The Enzyme Commission (EC) number is a numerical classification system for enzymes, developed by the International Union of Biochemistry and Molecular Biology (IUBMB). The EC number is assigned to enzymes based on their chemical reactions and the molecules (substrates) they act upon. Each EC number is unique and consists of four digits, separated by periods. These four digits appear in a hierarchical format, where each level encodes specific information. The first digit represents the type of chemical reaction (e.g. oxidation, hydrolysis, transfer), the second and third digits specify the substrate or group of substrates, and the fourth digit is used for further classification. The EC number is used to identify enzymes in databases and in scientific literature and can be useful for understanding the function of enzymes. The proposed dataset contains the scientific text that discusses a particular enzyme and its corresponding EC number. \\

% Most of the work in hierarchical text classification (HTC) can be categorized into two groups: global and local. In the global way of HTC, the model transforms the hierarchy into a flat structure and uses a single classifier for all the classes. This kind of model suffers from two major drawbacks. Firstly, it increases the number of classes in the classifier exponentially, which results in highly imbalanced data. Secondly, these methods capture the dependencies between the hierarchical classes in a very limited manner. These global models utilize Graph Convolution Networks (GCN) (cite), TreeLSTM (cite), Label correlation features (cite), hierarchical regularization (cite), and meta-learning (cite). On the other hand, the local way of HTC utilizes the hierarchical structure in a top-down manner. Information from the parent is transmitted to the children to capture the label semantics. These methods rely heavily on the label semantics and the dependency between different nodes in the hierarchy to encode richer information. Some of the earlier work overcomes the data imbalance issue of the global way by learning a top-down encoding utilizing information about the parent to arrive at the finer class. Another line of work by (cite) (cite) (cite) uses the joint representation of original text and labels to capture the interactions between them. All of the work so far in the field of HTC uses some kind of encoding framework for the text and label followed by classification. \\
 % \zc{no need for an extra blank line for each paragraph} 
 % \zc{use a paragraph to argue the drawbacks of existing methods that treat this problem as a supervised classification task. Namely, highlight the ``pain point'' that we are gonna address.} 

% In this end, motivated by the large-scale success of language models, we propose a generation-based framework for the task of HTC. To the best of our knowledge, we are the first ones to incorporate the autoregressive generation paradigm by leveraging the power of large language models in capturing contextual information during decoding. This framework is inspired by the encoding and transferring of the local information during the decoding to its next state. This framework captures the top-down hierarchy in an autoregressive way by generating the tag for the current level conditioned on the previous one. Language models like BART utilize the attention-based mechanism to encode a rich input text representation and leverage it during the decoding phase to capture the hierarchical structure in the labels. (cite) (cite) (cite) has shown that an effective pretraining strategy can largely influence the performance of the generation model on downstream tasks. The pretraining strategy can be viewed broadly using two lenses. Firstly, (cite) (cite) showed that the relevance of the pretraining task to the downstream task hugely boosts the performance on the downstream task. Secondly, (cite)(cite)(cite) showed the crucial role played by the dataset used to pretrain the model. In this work, we leverage both these views to propose a novel pretraining strategy using related weakly supervised data to jointly encode the input text and weakly supervised labels. After pretraining the model, we used the proposed MODEL-NAME to fine-tune the generation model on the specific dataset. We also employ a novel constraint decoding strategy using the prior information about the label hierarchy. \\

% The proposed dataset, ENZYME, is very imbalanced. There are a lot of enzyme classes having only a handful number of examples in the training set. We refer to these low-frequency classes as long-tailed classes. The proposed model is able to outperform the baselines on these long-tailed classes. In a similar light, the biomedicine domain has a very high dearth of human-curated data. This is because of the great expertise required in the subject and the cost of annotation. We explore the performance of all models for scenarios where there are only a few training labels present for all classes. These sets of experiments have a huge relevance in the field of biomedicine. \\
 % \zc{as a general comment, you need to make your paragraphs shorter} 

The major contributions of this paper are:
\begin{itemize}
    \item We propose a hierarchical text classification approach by modeling it as a generation problem. The generation model is able to capture the hierarchy in an autoregressive way, where the output from the previous time steps is used to predict the output for the next time step.
    \item We design an effective pretraining task by leveraging additional in-domain data to improve the model's performance. We also explore a constrained decoding strategy to generate more coherent labels.
    \item We demonstrate the excellence of our proposed approach on classes that are scarce by nature. Our model beats the baseline models for cases where only a minimal number of examples were used during training.
    \item We also propose a new dataset, ENZYME, containing 30523 full-text PubMed articles and their corresponding Enzyme Commission (EC) numbers which follow a deep hierarchical structure. \yue{It is not clear about the uniqueness of this dataset, and whether it can be considered a novelty since there are too many hierarchical text classification datasets already (as mentioned in Lines 56-60).}
\end{itemize}

